Zandpack: A General Tool for Time-dependent Transport Simulation of Nanoelectronics

The auxiliary mode approach to time-dependent open quantum system calculations is implemented and refined to yield a feasible computational approach to simulate nanostructures far from equilibrium. It is done by a careful diagonalization of the electrode level-width function, and provides an efficient approach which can simulate large, open systems at the level of time-dependent density functional theory. The approach, as given in this work, is implemented in the new open-source code Zandpack. The framework is applied to three systems perturbed by the same THz electromagnetic field pulse-form: 1) A Hubbard model for hydrogen on graphene is used to calculate spin-currents, mutual information, spin-transitions, and a pump-probe setup. 2) An armchair graphene nanoribbon (AGNR) probed by a metal tip showing electrons excited from the valence band of the AGNR into the tip via electron-electron interactions. 3) A gold break-junction is modeled with various gap distances, and displays behavior that is more different from the adiabatic case as the gap widens. In the examples 2 and 3, we develop and use a general linearization scheme for time-dependent open system calculations, which utilizes the DFTB+ or SIESTA codes.

==> Res/Results_P2_2.tex <==
\subsection{DFTB+ Interface: Aluminum break junction driven by THz Field}
Molecular break junctions can be realized in the laboratory using relatively simple equipment

==> Res/Results_P3.tex <==
\subsection{SIESTA Interface}

==> Res/Results_P4.tex <==
\section{Interface to the Mean-field Hubbard Code}
